Efficient Construction of Probabilistic Tree Embeddings

In this paper we describe an algorithm that embeds a graph metric $(V,d_G)$ on an undirected weighted graph $G=(V,E)$ into a distribution of tree metrics $(T,D_T)$ such that for every pair $u,v\in V$, $d_G(u,v)\leq d_T(u,v)$ and ${\bf{E}}_{T}[d_T(u,v)]\leq O(\log n)\cdot d_G(u,v)$. Such embeddings have proved highly useful in designing fast approximation algorithms, as many hard problems on graphs are easy to solve on tree instances. For a graph with $n$ vertices and $m$ edges, our algorithm runs in $O(m\log n)$ time with high probability, which improves the previous upper bound of $O(m\log^3 n)$ shown by Mendel et al.\,in 2009. The key component of our algorithm is a new approximate single-source shortest-path algorithm, which implements the priority queue with a new data structure, the "bucket-tree structure". The algorithm has three properties: it only requires linear time in the number of edges in the input graph; the computed distances have a distance preserving property; and when computing the shortest-paths to the $k$-nearest vertices from the source, it only requires to visit these vertices and their edge lists. These properties are essential to guarantee the correctness and the stated time bound. Using this shortest-path algorithm, we show how to generate an intermediate structure, the approximate dominance sequences of the input graph, in $O(m \log n)$ time, and further propose a simple yet efficient algorithm to converted this sequence to a tree embedding in $O(n\log n)$ time, both with high probability. Combining the three subroutines gives the stated time bound of the algorithm. Then we show that this efficient construction can facilitate some applications. We proved that FRT trees (the generated tree embedding) are Ramsey partitions with asymptotically tight bound, so the construction of a series of distance oracles can be accelerated.

==> FRT-ADO.tex <==
\section{FRT Based Approximate Distance Oracle}
\label{sec:FRT-ADO}

Here, we are going to prove Theorem~\ref{prob3}.

Clearly the construction time for $O(\log n)$ FRT trees is $O(m\log^2 n+n \log^3 n)$. The storage for a single FRT tree is $O(n)$, and the distance query on a FRT tree is $O(1)$ using standard LCA query. The main goal here is to prove the $O(\log c)$ bound for distance approximation.

Suppose we want to query the distance between node $u$ and $v$. Now we want to prove the following lemma:
\begin{lemma}
For every pair of $u$ and $v$ that $u,v\in V$, the minimum of the tree distances in all FRT trees $T_1, T_2, \cdots, T_k$ where $k=O(\log n)$ is less than $O(\log c)$ times their actual distance w.h.p. More precisely,
$$\Pr\left[\min_{1\leq i\leq k}\left\{D_{T_i}(u,v)\right\}>O(\log c)\cdot d_G(u,v)\right]\leq n^{-\Omega(1)}.$$
\end{lemma}
\begin{proof}
Notice that during this proof, all of the constants are ignored. We also run experiments on variety of graphs that show the high quality of distance approximation.

Without loss of generality, assume that the shortest distance between $u$ and $v$ is 1. Suppose that the first difference on \cps s of $u$ and $v$ appears on the $(i+1)$-th level of a single FRT tree. This indicates that the LCA of $u$ and $v$ on this FRT tree is on the $i$-th level, and then the tree distance no more than $O(\beta\cdot 2^{\delta-i})$.

Now we try to analyze the possibility that the LCA of $u$ and $v$ is on the $i$-th level where $0\leq i<\delta$. Let the ancestors of $u$ and $v$ on the $(i+1)$-th level is $w_u$ and $w_v$. A necessary but not sufficient condition that the LCA of $u$ and $v$ is on the $i$-th level is that $w_u\ne w_v$ and either $d(u,w_u)\leq \beta\cdot 2^{\delta-i-1}< d(u,w_u)+1$ or $d(v,w_v)\leq \beta\cdot 2^{\delta-i-1}< d(v,w_v)+1$ holds; otherwise, assume $\pi(w_u)<\pi(w_v)$, then $w_u$ also dominates $v$ on the $(i+1)$-th level and this leads to a contradiction.

Denote $w_j$ as the ancestor of $u$ on the $j$-th level. The next step is to compute the probability that any $w_j$ ($j<i$), we have $d(u,w_i)\leq \beta\cdot 2^{\delta-j+1}< d(u,w_j)+1$ holds. Define $n_j$ be the number of vertices that their distances to $u$ is less than $\beta\cdot 2^{\delta-j+1}$, and we know that $n_j\leq (c+1)n_{j+1}$. Let $X_j$ be the set of dominant vertices of $u$ whose distances to $u$ are in $\left(\beta\cdot 2^{\delta-j-1},\beta\cdot 2^{\delta-j}\right]$, i.e. the range of the $i$-th level of the FRT tree, and we have:
$$\Pr\left[\left|X_j\right|>c_j\log c\right]\leq{\E(|X_j|)\over c_j\log c}={1\over c_j\log c}\sum_{k=n_{j+1}+1}^{n_j}{1\over k}\leq{1\over c_j}$$
using Markov's inequality. Here $c_j$ is some constant discussed later.

Now we analyze the probability that at least one of the dominant vertices in $X_j$ fall into the \emph{critical} range that can possibly cause a larger distance approximation, which is $\left(\beta\cdot 2^{\delta-j}-1,\beta\cdot 2^{\delta-j}\right]$.
Since $\beta$ is chosen randomly, each element in $X_j$ falls into the range with probability of no more than $1\over \beta\cdot 2^{\delta-j-1}$.
Therefore, when there are no more than $c_j\log c$ elements in $X_j$, by taking the union bound, at least one of the dominant vertices in $X_j$ fall into the range is no more than $c_j\log c\over \beta\cdot 2^{\delta-j-1}$.

Here we give a definition that a specific level $j$ in an FRT tree is ``good'' for vertex $u$ if and only if the number of dominant vertices of $u$ on $j$-th level of the FRT tree is less than $c_j\log c$, and none of the dominant vertices in $X_j$ fall into the critical range; otherwise, we call this level to be ``bad''.
The reason to define this is because, if the top $l$ levels are all good for a pair of vertices $u$ and $v$, then the LCA of this pair will not be in the top $l$ levels (from the 0-th level to the $(l-1)$-th level) of the FRT tree.

By taking union bound we know that:
$$\Pr\left[{\tx{``the~}} j{^{\rm{th}}\tx{~level~is~bad''}}\right]\leq {1\over c_j}+{c_j\log c\over \beta\cdot 2^{\delta-j-1}}$$

Thus the possibility on the top $l$ levels are all good is:
$$\Pr\left[{\tx{``top~}} l {\tx{~levels~are~all~good''}}\right]\geq 1-\sum_{j=1}^{l}\left({{1\over c_j}+{c_j\log c\over \beta\cdot 2^{\delta-j-1}}}\right)$$
again taking union bound.

Let $l=\delta-\log\log c-12$ and $c_j=24\cdot 1.5^{l-j}$, we further have:
$$\Pr\left[{\tx{``top~}} l {\tx{~levels~are~all~good''}}\right]\geq 1-\sum_{j=1}^{l}\left({{1\over 24\cdot 1.5^{l-j}}+{24\cdot 1.5^{l-j}\log c\over \beta\cdot 2^{\delta-j-1}}}\right)$$
$$=1-{1\over 8}\left(1+8\cdot{192\log c\over\beta\cdot 2^{\delta-l}}\right)>1-\left({1\over 8}\left(1+{\log c\over2^{\log\log c}}\right)\right)={3\over 4}$$

For the other vertex $v$, similar result holds, so the probability that both vertices on the top $l$ levels are good is at least $1\over 2$, which indicates that the probability that the LCA of this vertex pair is not in the top $l$ level is no more than $1\over 2$.
\hide{From the definition of \emph{``good''} we know that if either $u$ or $v$ is bad on the $j$-th level, we can induce that $u$ and $v$ have different ancestors on $j$-th level, which is equivalent to that if $u$ and $v$ are both good on the $j$-th level, they should share the ancestor on the $j$-th level. Thus:
\begin{align*}
&\Pr[{\rm{The~LCA~of~}}u{\rm{~and~}}v{\rm{~is~not~on~the~top~}}l{\rm{~levels}}]\\
\ge&\Pr[u{\rm{~and~}}v{\rm{~share~ancestors~on~the~top~}}l{\rm{~levels}}]\\
\ge&\Pr[{\rm{On~each~of~the~top~}}l{\rm{~levels~}}u{\rm{~and~}}v{\rm{~are~both~good}}]\\
\ge&\frac{1}{2}
\end{align*}}

Hence, if we use $\Theta(\log n)$ FRT trees, the probability that in all of them $u$ and $v$ have LCA on the top $l$ levels is $(1/2)^{\Theta(\log n)}=n^{-\Theta(1)}$. By the distance property of an FRT tree, if the LCA of two tree nodes is not on the top $l$ levels, the maximum tree distance is no more than $8\cdot \beta\cdot2^{\delta-l-1}=O(2^{\log\log c})=O(\log c)$.
\end{proof}

\section{Experiments for FRT-Tree Based Approximate Distance Oracles}
\label{sec:exp}

In this section, we illustrate the experiment settings, implementation, and result analysis in details for the FRT-tree Based Approximate Distance Oracles.

In our experiment, we use 5 types of graphs, including 1D grids with 10,000 vertices, 2D grids with 100$\times$100 vertices and 3D grids with 22$\times$22$\times$22 vertices, a random slim graph with 10,000 vertices and 100,000 edges and diameter for 1,000, a random graph following power-low with 10,000 vertices and 100,000 edges and diameter for 10.
Meanwhile, for each type of graphs, we generate two sets of graphs, one unweighted and the other with weights for all edges uniformly randomly chosen from 1 to 1,000.
We believe that these graphs are representative for the real-world graphs that the shortest-distance queries are usually made on.
For example, the road networks are planar graphs and have similar graph properties to the 2D weighted grid.
The power-law graphs are generated using the preferential attachment process, which simulates the evolutions of social networks.

For each graph, we generated 32 FRT trees based on the exact \seq{}s of each graph and randomly picked 10,000 pairs of vertices for distance query. For each query, we considered the first several FRT trees constructed by our proposed algorithm and took the minimum of the tree distances, and we also used standard Dijkstra algorithm to compute the exact shortest distance as ground truth.
Since to compute the exact shortest distance by the standard Dijkstra algorithm is less efficient, we only pick such small number of queries so that the overall running time for the experiments is endurable.
The FRT trees are compressed to no degree-2 vertices, and we set the weight of each original edge to be the actual distance of the shortest path between the two vertices, stored in the \seq{}s of the graph.

The quality of approximation is measured by two indicators: the average approximation, which is the average stretch of all queries on a specific graph, and the worst approximation, which is the maximum stretch of all queries.

The results are shown in Table 1. We can find that both the average approximation and the worst approximation are very small on all the graphs. 8 FRT trees are able to provide average approximation within $20\%$ error on graphs with large diameter, and $50\%$ error with small diameter. The errors further decrease to $10\%$ and $35\%$ using 32 FRT trees, and for the worst approximation, the stretch is about 2 on graphs with small diameters and about 3 on graphs with large diameters. Notice that ADOs with theoretical bounds need $O(n^{1.5})$ space to provide 3-approximation, while our new algorithm only uses near-linear storage space.
Meanwhile, this method is easy to program, and fast and efficient on preprocessing and querying.

In order to better understand the trend of these indicators, we plot the graph for average approximation and worst approximation for each graph, which are shown in Figure~1.

\begin{table}[th!]
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\centering
\begin{tabular}{l@{~~}||r@{~~}r@{~~}r@{~~}r@{~~}r@{~~}r||r@{~~}r@{~~}r@{~~}r@{~~}r@{~~}r}
\hline
\multirow{2}{*}{Number of trees} & \multicolumn{6}{c||}{Average approximation} & \multicolumn{6}{c}{Worst approximation} \\
\cline{2-13}
 &          1 &          2 &          4 &          8 &         16 &         32 &          1 &          2 &          4 &          8 &         16 &         32 \\
 \hline\hline

1D-grid (unweighted)
&       1.41 &       1.14 &       1.07 &       1.01 &       1.00 &       1.00 &      90.45 &      51.30 &       6.84 &       3.24 &       1.89 &       1.05 \\

1D-grid (weighted)
&       1.42 &       1.14 &       1.06 &       1.01 &       1.00 &       1.00 &      66.45 &      14.81 &       6.15 &       2.58 &       1.50 &       1.00 \\

2D-grid (unweighted)
&       1.46 &       1.35 &       1.22 &       1.11 &       1.06 &       1.02 &      16.67 &      11.33 &      11.33 &       6.00 &       2.76 &       2.14 \\

2D-grid (weighted)
&       1.45 &       1.36 &       1.25 &       1.14 &       1.08 &       1.03 &      27.33 &       9.72 &       5.10 &       4.33 &       2.80 &       1.74 \\

3D-grid (unweighted)
&       1.66 &       1.54 &       1.38 &       1.18 &       1.11 &       1.06 &      26.00 &      10.00 &      10.00 &       5.00 &       3.00 &       2.33 \\

3D-grid (weighted)
&       1.75 &       1.57 &       1.44 &       1.23 &       1.17 &       1.12 &      21.13 &       9.25 &       6.45 &       3.39 &       2.65 &       2.11 \\
\hline

Slim (unweighted)
&       1.39 &       1.14 &       1.07 &       1.02 &       1.00 &       1.00 &      64.21 &      16.24 &       5.77 &       2.50 &       2.50 &       2.00 \\

Slim (weighted)
&       1.42 &       1.14 &       1.07 &       1.02 &       1.01 &       1.00 &      62.30 &      29.13 &       6.88 &       4.00 &       2.12 &       1.55 \\

Power-law (unweighted)
&       2.05 &       1.77 &       1.63 &       1.55 &       1.45 &       1.37 &       4.50 &       4.00 &       3.50 &       3.50 &       3.00 &       3.00 \\

Power-law (weighted)
&       2.28 &       1.89 &       1.65 &       1.43 &       1.32 &       1.21 &      13.15 &       4.85 &       4.85 &       4.54 &       3.31 &       3.31 \\
\hline
\end{tabular}

\caption{Average approximation and worst approximation for all 10 graphs using 1, 2, 4, 8, 16, and 32 FRT trees.}\label{table}
\end{table}

\begin{figure}[!th]
\centering
\vspace{-0.25in}
\subfigure[The average approximation on \textbf{unweighted} 1D, 2D and 3D grids]{
\begin{minipage}[t]{0.43\columnwidth}
\centering
\includegraphics[width=0.95\columnwidth]{figs/res_grid_average_unweighted.pdf}
\end{minipage}
}~~~~~
\subfigure[The worst approximation on \textbf{unweighted} 1D, 2D and 3D grids]{
\begin{minipage}[t]{0.43\columnwidth}
\includegraphics[width=0.95\columnwidth]{figs/res_grid_worst_unweighted.pdf}
\end{minipage}
}\\
\vspace{-0.14in}
\subfigure[The average approximation on \textbf{weighted} 1D, 2D and 3D grids]{
\begin{minipage}[t]{0.43\columnwidth}
\centering
\includegraphics[width=0.95\columnwidth]{figs/res_grid_average_weighted.pdf}
\end{minipage}
}~~~~~
\subfigure[The worst approximation on \textbf{weighted} 1D, 2D and 3D grids]{
\begin{minipage}[t]{0.43\columnwidth}
\includegraphics[width=0.95\columnwidth]{figs/res_grid_worst_weighted.pdf}
\end{minipage}
}\\
\vspace{-0.14in}
\subfigure[The average approximation on \textbf{unweighted} synthetic slim and power-law graphs]{
\begin{minipage}[t]{0.43\columnwidth}
\centering
\includegraphics[width=0.95\columnwidth]{figs/res_syn_average_unweighted.pdf}
\end{minipage}
}~~~~~
\subfigure[The worst approximation on \textbf{unweighted} synthetic slim and power-law graphs]{
\begin{minipage}[t]{0.43\columnwidth}
\includegraphics[width=0.95\columnwidth]{figs/res_syn_worst_unweighted.pdf}
\end{minipage}
}\\
\vspace{-0.14in}
\subfigure[The average approximation on \textbf{weighted} synthetic slim and power-law graphs]{
\begin{minipage}[t]{0.43\columnwidth}
\centering
\includegraphics[width=0.95\columnwidth]{figs/res_syn_average_weighted.pdf}
\end{minipage}
}~~~~~
\subfigure[The worst approximation on \textbf{weighted} synthetic slim and power-law graphs]{
\begin{minipage}[t]{0.43\columnwidth}
\includegraphics[width=0.95\columnwidth]{figs/res_syn_worst_weighted.pdf}
\end{minipage}
}
\vspace{-0.1in}
\caption{The approximation on different types of graphs using 1 to 32 FRT trees.}
\end{figure}






\hide{
\begin{figure}[!th]
\centering
\subfigure[The Average Approximation]{
\begin{minipage}[t]{0.4\columnwidth}
\centering
\includegraphics[width=1\columnwidth]{figs/res_grid_average_weighted.pdf}
\end{minipage}
}
\subfigure[The Worst Approximation]{
\begin{minipage}[t]{0.4\columnwidth}
\includegraphics[width=1\columnwidth]{figs/res_grid_worst_weighted.pdf}
\end{minipage}
}
\caption{Stretch on \textbf{weighted} 1D, 2D and 3D grids using 1 to 32 FRT trees.}
\end{figure}

\begin{figure}[!th]
\centering
\subfigure[The Average Approximation]{
\begin{minipage}[t]{0.4\columnwidth}
\centering
\includegraphics[width=1\columnwidth]{figs/res_syn_average_unweighted.pdf}
\end{minipage}
}
\subfigure[The Worst Approximation]{
\begin{minipage}[t]{0.4\columnwidth}
\includegraphics[width=1\columnwidth]{figs/res_syn_worst_unweighted.pdf}
\end{minipage}
}
\caption{Stretch on \textbf{unweighted} synthetic slim and power-law graphs using 1 to 32 FRT trees.}
\end{figure}

\begin{figure}[!th]
\centering
\subfigure[The Average Approximation]{
\begin{minipage}[t]{0.4\columnwidth}
\centering
\includegraphics[width=1\columnwidth]{figs/res_syn_average_weighted.pdf}
\end{minipage}
}
\subfigure[The Worst Approximation]{
\begin{minipage}[t]{0.4\columnwidth}
\includegraphics[width=1\columnwidth]{figs/res_syn_worst_weighted.pdf}
\end{minipage}
}
\caption{Stretch on \textbf{weighted} synthetic slim and power-law graphs using 1 to 32 FRT trees.}
\end{figure}

\begin{figure}[th!]
\centering
  \includegraphics[width=0.45\columnwidth]{figs/Approximation_chain_2d_3d_0}~~~~
  \includegraphics[width=0.45\columnwidth]{figs/Worse_chain_2d_3d_0}\\
  \includegraphics[width=0.45\columnwidth]{figs/Approximation_chain_2d_3d_1}~~~~
  \includegraphics[width=0.45\columnwidth]{figs/Worse_chain_2d_3d_1}\\
  \includegraphics[width=0.45\columnwidth]{figs/Approximation_thin_fat_0}~~~~
  \includegraphics[width=0.45\columnwidth]{figs/Worse_thin_fat_0}\\
  \includegraphics[width=0.45\columnwidth]{figs/Approximation_thin_fat_1}~~~~
  \includegraphics[width=0.45\columnwidth]{figs/Worse_thin_fat_1}\\
\caption{The decrease of average approximation and worst approximation on each graph using 1 to 32 FRT trees.}\label{graphs}
\end{figure}
}



==> FRTADO.tex <==
\section{Simple FRT-Tree Based Approximate Distance Oracles}
\label{sec:FRTADO}

As stated in the previous sections, one of the most significant advantages to use FRT trees to construct approximate distance oracles is the simplicity of FRT trees in both theory and practice. In this section, we show a simple way to construct ADOs on a sparse graph $G=(V,E)$.  The  idea is simply to use $\Theta(\log n)$ FRT trees as a basic data structure, and each query is responded by querying all tree distances and taking the minimum value.
Theoretically we can show the following approximation bound for this distance oracle.

\hide{We analyze the approximation bound on doubling
space~\cite{karger2002}, and a measure $\mu$ on a metric space
$(X,d_x)$ is $c$-doubling if there is a constant $c > 0$ such that
$\mu(B(x,2r))\le c\mu(B(x,r))$. \guy{Is this repeating from the preliminaries.}}

\begin{theorem}
\label{prob3}
The approximate distance oracle by combining the queries on $\Theta(\log n)$ FRT trees uses $O(m\log^2 n)$ preprocessing time, $O(n\log n)$ space, provides $O(\log c)$-approximation w.h.p., and responds queries in $O(\log n)$ time, i.e.\ an $(O(m\log^2 n), O(n\log n),O(\log n),O(\log c))$-ADO.  Here, $c$ is the KR-expansion of the graph metric.
\end{theorem}

Clearly the construction time for $O(\log n)$ FRT trees is $O(m\log^2 n)$. The storage space for a single FRT tree is $O(n)$, and the distance query on a FRT tree is $O(1)$ using a standard LCA query. The proof of the $O(\log c)$ bound for distance approximation is provided in Section~\ref{sec:FRT-ADO} in the appendix.

Although the $O(\log c)$ bound is not particularly attractive theoretically, our main goal for this section is to show that, in practice this simple ADO works well on a variety of graph types.
In our experiment, we tested 5 types of graphs, including 1D grids, 2D grids, 3D grids, a random slim graph with large diameters, and a random graph obeying the power-low (social network graphs with low diameters).   We tested both weighted and unweighted cases on all types of graphs.

For each graph, we generate 32 FRT trees based on the exact \seq{}s of each graph and randomly pick 10,000 pairs of vertices
for distance queries.  Since to compute the exact shortest distance by
the standard Dijkstra algorithm is less efficient, we limit the number
of queries so that the overall running time for the experiments is
acceptable.

Detailed experiment settings and full version of result analysis can
be found in Appendix~\ref{sec:exp}, and here we only briefly
summarized some interesting conclusions.

We noticed that if we use 32 FRT trees for each graph in the
experiments, the average approximation (average stretch of all queries
on a specific graph) is no more than 1.4 and the geometric mean for
all types of graphs is only 1.07.  For the worst approximation (the
maximum stretch of all queries), the largest stretch of all queries is
3.3 and the geometric mean is 1.9.

We understand that this method does not work well on all graphs, especially on high-girth graphs, which are used to construct the $O(n^{1+1/k})$ lower bound for distance oracles.  However, for most of the real-world graphs (e.g. road networks that are usually planar graphs, social networks, etc.) for which shortest-distance queries are usually used for, this ADO with almost linear space and constant query time (32 LCA queries) seems to work well.
%, especially comparing to standard ADOs with theoretical bounds that need $O(n^{1.5})$ space to provide 3-approximation.
Lastly, the implementation of the approach is simple.  Our code is
only a few hundred lines of code and we implemented it within one
afternoon.


==> Ramsey.tex <==
\section{Efficient Hierarchical Ramsey Partition}
\label{sec:ramsey}
In this section, we prove introduce a new algorithm to generate a Ramsey partition with the same optimal bounds proposed in~\cite{Ramsey}. The main theorem for this section is:
\begin{theorem}
\label{thm:Ramsey}
The partition tree $\{\mathscr{E}_k\}_{k=0}^{\infty}$ of a metric space $(X, d_X)$ from Algorithm~\ref{algo:ramseyADO} is a Ramsey partition, with asymptotically tight bound of $\alpha=\Omega(\gamma)$. Furthermore, such partition tree on a sparse graph can be generated in $O(m\log n+n\log^2 n)$ time.
\end{theorem}

The differences between the partition tree in Algorithm~\ref{algo:ramseyADO} and the conventional process (introduced in \cite{Ramsey,FastCKR}) of a Ramsey partition based ADO in that when constructing the HST, we use the same random permutation in all levels instead of generating a new random permutation each round.

Recall the conversional process of a CKR Partition process. It accepts an $n$-point metric space $(X,d_X)$, a scale $\Lambda$, and yields a partition of $X$. During CKR Partition process, a random permutation $\pi$ representing the priority of each point will be generated thus every CKR Partition takes a different random permutation. Here our modification is to input one more parameter $\pi$ as the preprocessed random permutation. We call this process ``pseudo CKR Partition'' for the loss of the randomness of $\pi$. The pseudocode is shown in Algorithm \ref{algo:ckr}.

\begin{algorithm}[!th]
\caption{Pseudo CKR Partition}
\label{algo:ckr}
\textbf{Input}: an n-point metric space $(X,d_X)$, a scale $\Lambda>0$ and a random permutation of $[n]$ $\pi$\\
\textbf{Output}: partition $\mathscr{P}$ of $X$\\
    %\vspace{0.5em}
    \begin{algorithmic}[1]
    \STATE {$R\leftarrow$ real random in $\left[\frac{\Lambda}{4},\frac{\Lambda}{2}\right]$}
    \STATE {$\ell\leftarrow$ a list of length $n$ containing $[n]$ generated by the priority in $\pi$, i.e., $\ell_i=j$ iff $\pi_j=i$.}
    \FOR {$i\leftarrow 1$ to $n$}
        \STATE {$C_i\leftarrow B_X(x_{\ell_i},R)\backslash \bigcup_{j=1}^{i-1}C_j$}
    \ENDFOR
    \STATE {$\mathscr{P}\leftarrow\{C_1,\dots,C_n\}\backslash \{\emptyset\}$}
    \RETURN {$\mathscr{P}$}
   \end{algorithmic}
%    \vspace{.5em}
\end{algorithm}

Now we can get the partition tree based on this partition as Algorithm~\ref{algo:ramseyADO}.

\begin{algorithm}[!th]
\caption{Pseudo Ramsey-ADO}
\label{algo:ramseyADO}
\textbf{Input}: an n-point metric space $(X,d_X)$, approximation factor $\alpha\ge 1$.\\
\textbf{Output}: a partition tree of $X$: $\{\mathscr{E}_j\}_{j=0}^{\infty}$ \\
    %\vspace{0.5em}
    \begin{algorithmic}[1]
    \STATE {$\phi \leftarrow \mb{diam}(X)$}
    \STATE {$\mathscr{P_0}\leftarrow\{X\}$.}
    \STATE {$\mathscr{E_0}\leftarrow\mathscr{P_0}$.}
    \STATE {$k\leftarrow 1$}
    \REPEAT
        \STATE {$\mathscr{P}_{k}\leftarrow \mb{\textbf{CKR Partition}}(X,d_X),8^{-k}\phi,\pi$}
        \STATE {$\mathscr{E}_k\leftarrow\{C\cap C'|C\in \mathscr{E}_{k-1},C'\in \mathscr{P}_k\}$//refinement}
        \STATE {$k\leftarrow k+1$}
    \UNTIL {$|\mathscr{E}_{k-1}|=|X|$}
    \RETURN {$\{\mathscr{E}_k\}_{j=0}^{k-1}$}
   \end{algorithmic}
%    \vspace{.5em}
\end{algorithm}

Next, we will prove that even though we do not change random permutation each round, the algorithm shown in Algorithm \ref{algo:ramseyADO} still provides a Ramsey partition.

\begin{lemma}
\label{l1}
Given an $n$-point metric space $(X, d_X)$. Let $\mathscr{P}$ be a random CKR partition of $(X, d_X)$ created with scale $\Lambda>0$. Then for every $0\le t\le \Lambda/8$ and every $x\in X$,
$$Pr[B_X(x,t)\subseteq \mathscr{P}(x)]\ge\left(\frac{|B_X(x,\Lambda/8)|}{|B_X(x,\Lambda)|}\right)^{\frac{16t}{\Lambda}}.$$
\end{lemma}
\begin{proof}
Let $\pi,R$ be the random parameters chosen in the creation of $\mathscr{P}$ using Algorithm \ref{algo:ckr} (\textbf{CKR Partition}). For every $r\in [\Lambda/4,\Lambda/2]$, $$Pr[B_X(x,t)\subseteq \mathscr{P}(x)|R=r]\ge\frac{|B_X(x,r-t)|}{|B_X(x,r+t)|}.$$
This is because if $R=r$, then the triangle inequality implies that if in the random order induced by the partition $\pi$ on the points of the ball $B_X(x,r+t)$ the minimal element is from the ball $B_X(x,r-t)$, then $B_X(x,t)\subseteq\mathscr{P}(x)$. The aforementioned event happens with probability $\frac{|B_X(x,r-t)|}{|B_X(x,r+t)|}$.
\begin{align}
\nonumber
Pr[B_X(x,t)\subseteq \mathscr{P}(x)]&\ge \frac{4}{\Lambda}\int_{\Lambda/4}^{\Lambda/2}\frac{|B_X(x,r-t)|}{|B_X(x,r+t)|}dr\\
\label{l1proof}
&\ge\left[\frac{|B_X(x,\Lambda/8)|}{|B_X(x,\Lambda|)|}\right]^{\frac{16t}{\Lambda}}
\end{align}
A complete proof of (\ref{l1proof}) is provided in \cite{Ramsey}.
\end{proof}

\begin{lemma}
\label{random}
Assume we have a random permutation $\pi$ of length $n$. By randomly removing $m$ numbers in $\pi$ we generate a new list of length $n-m$, denoting as $\pi'$. The total order of $\pi'$ is a random permutation of length $n-m$.
\end{lemma}
\begin{proof}
It is obvious that if only one number is removed from $\pi$, and all numbers greater than it is decreased by $1$, the new list is still a random permutation of length $n-1$. Then this lemma could be proven by induction.
\end{proof}

\begin{lemma}
\label{l2}
Given $\alpha\ge 1$ and an n-point metric space $(X,d_X)$. Let $\{\mathscr{E}_k\}_{k=0}^{\infty}$ be a partition tree of $X$, created as described in Algorithm \ref{algo:ramseyADO}. Then for every $x\in X$,$$Pr\left[\forall k\in \mathbb{N}, B_X\left(x,\frac{8^{-k}\phi}{16\alpha}\right)\subseteq \mathscr{E}_k(x)\right]\ge |X|^{-\frac{1}{\alpha}}$$
\end{lemma}
\begin{proof}
For every $x\in X$ and every $k>0$ we have $\mathscr{E}_k=\mathscr{E}_{k-1}(x)\cap \mathscr{P}_k(x)$. Thus one proves inductively that
$$\forall k \in \mathbb{N},B_X\left(x,\frac{8^{-k}\phi}{16\alpha}\right)\subseteq\mathscr{E}_k(x) \Longrightarrow \forall k\in \mathbb{N},B_X\left(x,\frac{8^{-k}\phi}{16\alpha}\right)\subseteq \mathscr{E}_k(x)$$

Thus,

$$Pr\left[\forall k\in \mathbb{N},B_X\left(x,\frac{8^{-k}\phi}{16\alpha}\right)\subseteq\mathscr{E}_k(x)\right]\ge Pr\left[\forall k\in \mathbb{N},B_X\left(x,\frac{8^{-k}\phi}{16\alpha}\right)\subseteq\mathscr{P}_k(x)\right]$$

Notice that when $k$ is large enough, $Pr\left[\forall k\in \mathbb{N},B_X\left(x,\frac{8^{-k}\phi}{16\alpha}\right)\subseteq\mathscr{P}_k(x)\right]$ will be $1$ because $\mathscr{P}_k(x)$ is sufficiently small that there is only one point in it, i.e., $x$ itself. In that case, $Pr\left[\forall k\in \mathbb{N},B_X\left(x,\frac{8^{-k}\phi}{16\alpha}\right)\subseteq\mathscr{P}_k(x)\right]\equiv 1$. Assume that $\kappa=\arg \max_{k} Pr\left[\forall k\in \mathbb{N},B_X\left(x,\frac{8^{-k}\phi}{16\alpha}\right)\subseteq\mathscr{P}_k(x)\right]<1$.

Consider the largest circle centered at $x$, i.e., when $k=\kappa$. The probability of $B_X\left(x,\frac{8^{-\kappa}\phi}{16\alpha}\right)$ to be inside $\mathscr{P}(x)$, according to Lemma \ref{l1}, is larger than the probability that in the random order induced by the partition $\pi$, on the points of the ball $B_X(x,r+t)$, the minimal element is from the ball $B_X(x,r-t)$, i.e., it is larger than $\left[\frac{|B_X(x,8^{-\kappa-1}\phi|)}{|B_X(x,8^{-\kappa}\phi)|}\right]^{\frac{1}{\alpha}}$.

Next, we remove all the points in the largest circle and consider the next out-most circle, i.e., when $k=\kappa-1$. Notice that $\pi$ is a random permutation, the for every point $x$, the nodes which are furthest from it (i.e., in the largest circle) are assigned completely random labels. According to Lemma \ref{random}, we know that the total order of the labels of the rest points is still a random permutation. Thus when looking at the $(\kappa-1)^{th}$ circle, the probability of $B_X\left(x,\frac{8^{-(\kappa-1)}\phi}{16\alpha}\right)$ to be inside $\mathscr{P}(x)$, is independent with the previous circles, and is still larger than $\left[\frac{|B_X(x,8^{-\kappa-1}\phi|)}{|B_X(x,8^{-\kappa}\phi)|}\right]^{\frac{1}{\alpha}}$, and so forth. Thus we have:
\begin{align*}
Pr\left[\forall k\in \mathbb{N},B_X\left(x,\frac{8^{-k}\phi}{16\alpha}\right)\subseteq\mathscr{E}_k(x)\right]&\ge Pr\left[\forall k\in \mathbb{N},B_X\left(x,\frac{8^{-k}\phi}{16\alpha}\right)\subseteq\mathscr{P}_k(x)\right]\\
&=\prod_{k=0}^{\infty} Pr\left[B_X\left(x,\frac{8^{-k}\phi}{16\alpha}\right)\subseteq\mathscr{P}_k(x)\right]\\
&=\prod_{k=0}^{\kappa} Pr\left[B_X\left(x,\frac{8^{-k}\phi}{16\alpha}\right)\subseteq\mathscr{P}_k(x)\right]\\
&\ge\prod_{k=0}^{\kappa} \left[\frac{|B_X(x,8^{-\kappa-1}\phi|)}{|B_X(x,8^{-\kappa}\phi)|}\right]^{\frac{1}{\alpha}}\\
&=|B_X(x,\phi)|^{-\frac{1}{\alpha}}\\
&=|X|^{-\frac{1}{\alpha}}
\end{align*}
\end{proof}

%\begin{proof}
%From Lemma \ref{l2} and the definition of Ramsey partition we can directly prove the theorem.
%\end{proof}




==> cps-FRT.tex <==
\section{FRT Construction Based on \CPS s}
\label{app:FRT}

To start with, we first illustrate how to construct an FRT tree based on the \pars~s $\sigma_{\pi,\beta}$ of a graph.

Define $\mb{prefix}\left(\sigma_{\pi,\beta}^{(v)},i\right)$ to be the $(i+1)$-dimensional vector that contains the dominant vertices in the first $i$ levels, which just takes the first $i+1$ elements in $\sigma_{\pi,\beta}^{(v)}$. The FRT tree $T$ generated by $\sigma_{\pi,\beta}^{(v)}$ is the tree that contains:

\begin{itemize}
  \item Vertices: Let $L_i=\{\mb{prefix}\left(\sigma_{\pi,\beta}^{(v)},i\right)\,|\,v\in V\}$ for all $i$ from $0$ to $\delta$, be the $i$-th level in the tree. The vertices of $T$ are the combination of all levels, i.e. $V(T)=\cup_iL_i$.
  \item Edges: Edges are from $L_i$ to $L_{i+1}$ for $0\leq i<\delta$. More specifically, an edge $(x,y)$ where $x\in L_i$ and $y\in L_{i+1}$ is in $E(T)$ if and only if $x$ is a prefix of $y$.
\end{itemize}

For a standard FRT tree, the weight of the edges in the $i$-th level is set to be $\beta\cdot 2^{\delta-i}$.  If a more accurate approximation is required (in Section~\ref{sec:FRTADO}), the weight of an edge $(u,v)$ can be the actual distance between the two vertices that corresponds to the two endpoints of this edge, which is already precomputed and stored in $d(u,v)$.

Notice that the way to construct such FRT tree is similar to the process to build a trie, where we treat each vertex as a string based on the alphabet $[n]$. The space and time complexity of such process is $O(n\delta)$. Actually, the strings for each vertex is stored in $\sigma_{\pi,\beta}^{(v)}$, and the compressed version is in $\bar{\sigma}_{\pi,\beta}^{(v)}$.

To further accelerate the process to construct FRT trees and reduce space usage since $\delta$ can be arbitrarily large, we use the concept of a
\emph{compacted FRT tree}\,\cite{Kanat}, which is obtained by contracting all degree-2 internal nodes of an FRT tree. The weight for a new edge is the sum of the weights of the merged edges, so the compaction preserves the distance between every pair of leaves.

It is interesting to point out that a compacted FRT tree is actually a Patricia tree on the input of the \cps. Clearly the space to store a compacted FRT tree is $O(n)$ since interior nodes are strictly less than leaf nodes. Since only $O(\log n)$ w.h.p. nodes are in the \cps~of each vertex, any efficient algorithm to construct Patricia tree leads to an $O(n\log n)$ time complexity.

Lastly, we show the distance preserving properties of our new efficient FRT construction algorithm.

\begin{lemma}
For all $u,v\in V$,
$$d_G(u,v)\leq d_T(u,v)$$
and
$$\E\left[d_T(u,v)\right]\leq O(\log n)\cdot d_G(u,v)$$
where $d_T(u,v)$ is measured by adding the weights from the leaf nodes corresponding to $u$ and $v$ to their lowest common ancestor.
\end{lemma}

This lemma is previously proved in Lemma 3.3 and Lemma 3.4 in~\cite{Kanat}.



==> future.tex <==
\section{Future Works}

In this section we introduced a number of theorems that we have already proved, but due to the limited time, we have not yet finished them on the current version. Such theorems include:

\begin{theorem}
Given a graph $G=(V,E)$ with $n$ vertices and $m$ edges, with $O(mn^\delta)$ work and $O(d)$ span in preprocess\,\cite{Cohen} where $\delta=\Omega(1/\log\log n)$ and $d=\left(\log n\over \epsilon\right)^{1/\delta^2}$, a partition tree can be generated using $O(md\log n)$ work and $O(d\log n)$ span on a PRAM machine.
\end{theorem}
This theorem is able to provide a parallel version of all of the Ramsey partition based ADO.

